Learning Manifolds for Sequential Motion Planning

Motion planning with constraints is an important part of many real-world robotic systems. In this work, we study manifold learning methods to learn such constraints from data. We explore two methods for learning implicit constraint manifolds from data: Variational Autoencoders (VAE), and a new method, Equality Constraint Manifold Neural Network (ECoMaNN). With the aim of incorporating learned constraints into a sampling-based motion planning framework, we evaluate the approaches on their ability to learn representations of constraints from various datasets and on the quality of paths produced during planning.

==> RSS2020_TAMP Workshop_SMP_Learning/abstract.tex <==
\begin{abstract}
% We expand on the previous work in constrained robot motion planning on manifold sequences.
% We consider the case where a manifold constraint is not known analytically.
% Instead, we have used techniques from machine learning to learn representations of the constraints from data. 
% We compare several approaches for multiple robotic datasets,
% and we discuss how to incorporate the learned constraints into an existing planning framework.
% We conclude with insights learned and next steps.
Motion planning with constraints is an important part of many real-world robotic systems. 
In this work, we study manifold learning methods to learn such constraints from data.
We explore two methods for learning implicit constraint manifolds from data: Variational Autoencoders (VAE), and a new method, {\ecmnnlong} ({\ecmnn}). With the aim of incorporating learned constraints into a sampling-based motion planning framework, we evaluate the approaches on their ability to learn representations of constraints from various datasets and on the quality of paths produced during planning.
\end{abstract}

==> RSS2020_TAMP Workshop_SMP_Learning/background.tex <==
\section{Background on Sequential Manifold Planning}
\label{sec:background}
We focus on learning manifolds that describe kinematic robot tasks. We aim to integrate these learned manifolds into the sequential manifold planning (SMP) framework proposed in \citet{englert2020sampling}.
SMP considers kinematic motion planning problems in a configuration space $\configspace \subseteq \Re^{\dimambient}$. A robot configuration 
% $q\in C$ 
$\jointposition \in \configspace$
describes the state of one or more robots with 
% $k$ 
$\dimambient$
degrees of freedom in total.
%
A manifold 
% $M$ 
$\constraintmanifold$
is represented as an equality constraint 
% $h_{M}(q)=0$ 
$\constraintfunction(\jointposition) = \vct{0}$
where 
% $h_{M}(q) : \R^{k} \to \R^{l}$. 
$\constraintfunction: \Re^{\dimambient} \rightarrow \Re^{\dimconstraint}$
and $\dimconstraint$ is the dimensionality of the implicit manifold.
The set of robot configurations that are on a manifold 
% $M$ 
$\constraintmanifold$
is given by 
% $$C_{M} = \{q\in C ~|~ h_{M}(q) = 0\}\period$$
\mbox{$\onconstraintconfigspace = \{ \jointposition \in \configspace \mid \constraintfunction(\jointposition) = \vct{0} \}\period$}
%
SMP defines the planning problem as a sequence of 
% $n+1$ 
$(\numconstraintmanifold+1)$
such manifolds 
% $$\mathcal{M} = \{M_1, M_2, \dots, M_{n+1}\}$$
\mbox{$\mathcal{\constraintmanifold} = \{\constraintmanifold_1, \constraintmanifold_2, \dots, \constraintmanifold_{\numconstraintmanifold+1}\}$}
and an initial configuration 
% $q_\t{start}\in C_{M_1}$ 
$\jointposition_\t{start} \in \configspace_{{\constraintmanifold}_1}$ 
that is on the first manifold.
%
The goal is to find a path from 
% $q_\t{start}$ 
$\jointposition_\t{start}$ 
that traverses the manifold sequence 
% $\mathcal{M}$ 
$\constraintmanifoldsequence$
and reaches a configuration on the goal manifold 
% $M_{n+1}$. 
$\constraintmanifold_{\numconstraintmanifold+1}$. 
A path on the $i$-th manifold is defined as 
% $\tau_i : [0, 1] \to C_{M_i}$
$\tpath_i : [0, 1] \to {\onconstraintconfigspace}_{i}$
and 
% $J(\tau_i)$ 
$\cost(\tpath_i)$ 
is the cost function of a path
% $\mathcal{J} : \mathcal{T} \to \R_{\geq 0}$
$\costfunctional : \tpathspace \to \Re_{\geq 0}$
where 
% $\mathcal{T}$ 
$\tpathspace$ 
is the set of all non-trivial paths. The problem is formulated as an optimization over a set of paths 
% $\vct\tau = (\tau_1, \dots, \tau_{n})$ 
$\tpathset = (\tpath_1, \dots, \tpath_{\numconstraintmanifold})$ 
that minimizes the sum of path costs under the constraints of traversing 
% $\mathcal{M}$ 
$\constraintmanifoldsequence$ 
and of being collision-free:
% \begin{align} %
% 	\begin{alignedat}{2} %	
% 	\label{eq:smp_problem}
% 	&\vct\tau^{\star} = \argmin_{\vct\tau} \sum_{i=1}^n J(\tau_i) &&\\
% 	\st\quad &\tau_1 (0) = q_\t{start} &\\
% 	&\tau_i(1) = \tau_{i+1}(0)  &&\forall_{i=1,\dots,n-1} \\ 
% 	&C_{\t{free}, i+1} = \Upsilon(C_{\t{free}, i}, \tau_{i})~~~~ &&\forall_{i=1,\dots,n}\\
% 	&\tau_i(s) \in C_{M_i} \cap C_{\t{free}, i} &&\forall_{i=1,\dots,n}~ \forall_{s \in [0, 1]}\\
% 	&\tau_{n}(1) \in C_{M_{n+1}} \cap C_{\t{free}, n+1} &&
% 	\end{alignedat} %
% \end{align}
\begin{align} %
	\begin{alignedat}{2} %	
	\label{eq:smp_problem}
	&\tpathset^{\star} = \argmin_{\tpathset} \sum_{i=1}^{\numconstraintmanifold} \cost(\tpath_i) &&\\
	\st\quad &{\tpath}_1 (0) = {\jointposition}_\t{start} &\\
	&\tpath_i(1) = \tpath_{i+1}(0)  &&\forall_{i=1,\dots,\numconstraintmanifold-1} \\ 
	&\configspace_{\t{free}, i+1} = \freeconfigspaceoperator(\configspace_{\t{free}, i}, \tpath_{i})~~~~ &&\forall_{i=1,\dots,\numconstraintmanifold}\\
	&\tpath_i(s) \in {\onconstraintconfigspace}_{i} \cap \configspace_{\t{free}, i} &&\forall_{i=1,\dots,\numconstraintmanifold}~ \forall_{s \in [0, 1]}\\
	&\tpath_{\numconstraintmanifold}(1) \in {\onconstraintconfigspace}_{\numconstraintmanifold+1} \cap \configspace_{\t{free}, \numconstraintmanifold+1} &&
	\end{alignedat} %
\end{align}
%
% $\Upsilon$ 
$\freeconfigspaceoperator$
is an operator that describes the change in the free configuration space (the space of all configurations that are not in collision with the environment)
% $C_\t{free}$ 
$\configspace_\t{free}$ 
when transitioning to the next manifold. The SMP algorithm is able to solve this problem for a certain class of problems. It iteratively applies RRT${}^\star$ to find a path that reaches the next manifold while staying on the current manifold.
For further details of the SMP algorithm, we refer the reader to \citet{englert2020sampling}. 

In this paper, we employ data-driven algorithms to learn manifolds $M$ from data with the goal to integrate them into the SMP framework.
%
% maybe we don't need this section, if we beef up the intro paragraph a little
% or, maybe we include this but just explain how manifolds were represented before.
% TOOD: need to define h(q), C_M


==> RSS2020_TAMP Workshop_SMP_Learning/datasets.tex <==
\section{Datasets}
\label{sec:datasets}
We use a robot simulator (\citet{todorov2012mujoco}) to generate various datasets. For each dataset, we define $\constraintfunction(\jointposition)$ by hand and randomly sample points in the configuration space and project them onto the manifold. We use six datasets:
\begin{itemize}
    \item \textbf{Nav}: 2D point that has to stay close to a reference point. Defined as an inequality constraint. $N=15000$.
    \item \textbf{Sphere}: 3D point that has to stay on the surface of a sphere. $N=10000$.
    % renaming all 3DOF to "Plane" 
    \item \textbf{Plane}: Robot arm with 3 rotational DOFs where the end effector has to be on a plane. $N=999$.
    % renaming all 6DOF to "Orient"
    \item \textbf{Orient}: Robot arm with 6 rotational DOFs that has to keep its orientation upright (e.g., transporting a cup). $N=21153$.
    \item \textbf{Tilt}: Same as Orient, but here the orientation constraint is relaxed to an inequality constraint. $N=2000$.
    \item \textbf{Handover}: Robot arm with 6 rotational DOFs and a mobile base with 2 translational DOFs. The manifold is defined as an equality constraint that describes the handover of an object between the two robots. $N=2002$.
\end{itemize}



\begin{comment}
\subsection{Data production}
% TODO: this is only accurate for equality constraints. Need to update for the
% Tilt and Nav datasets. 
Data for this problem are produced in simulation following
\citet{englert2020sampling}: Constraints are written in the form of equalities in
configuration space. Configurations are sampled randomly in valid configuration
space, and they are subsequently projected onto the constraint manifold using
iterative gradient descent (\citet{kingston2018sampling}). In the case that
projection fails to produce a valid point (e.g., because of local minima
encountered in the configuration space), the sample is rejected and a new point
is sampled.

Configurations that do not adhere to the constraints (``off-manifold data'') can
be computed easily by randomly sampling the configuration space, evaluating the
constraint function at that point, and, if desired, rejecting if it is below a
threshold. Alternatively, near-on-manifold configurations may be kept as a way
to introduce noise to the dataset. In general, the randomly selected
configurations will have probability 0 of being on the manifold, since the
constraint defines an implicit set of measure zero in the configuration space,
and thus producing a large off-manifold dataset can be simple.

The data is represented as an $n$ by $d$ matrix, where $n$ is the number of
samples (configurations) and $d$ is the dimension (DOF) of the configuration
space. Note that for a simple robotic scenario, the environment could consist of
a single arm with just 3 DOFs. In this case, the data matrix is $n$ by $3$.
However, in most practical applications, robots will each have at least 6 and
possibly many more DOFs. In this case, the data matrix will be of size $n$ by
$\sum_a d_a$ where $d_a$ denotes the number of DOFs of robot $a$ in the
environment.

We learn models for the following constraints:
\begin{enumerate}
\item 2DOF: Stay within 1 unit radius of a point of interest (Nav)
\item 3DOF: Stay on a sphere (Sphere)
\item 3DOF: Keep end effector on a 2D line (3DOF)
\item 6DOF: Keep end effector at a specific orientation (6DOF)
\item 6DOF: Keep end effector within a small deviation of an orientation (Tilt)
\item 8DOF: Pass an object between two robots (Handover)
\end{enumerate}

\subsection{Nav dataset}
\label{nav_dataset_section}
This dataset is a 2D inequality constraint where the position of a robot represented as a 2-dimensional vector should stay within a certain distance of a point of interest. This scenario is meant as a simple example of a navigation task where a robot's motion plan may be restricted by the communication limitations of a central tower. The data matrix is of size % TODO fill in the size

\subsection{Sphere dataset}
In the Sphere dataset, the constraint is a geometric one, constraining the configuration to lie on the surface of a sphere in 3D space. The data matrix is of size % TODO fill in the size

\subsection{3DOF dataset}
In the ``3DOF dataset", the constraint is to maintain the end effector of a
planar 3-link robot arm on a line. The data matrix is of size $999$ by
$3$. 

% See figures \ref{fig_3dof_generate} and \ref{fig_6dof_generate} for some sample poses whose configurations make up the two datasets. 

\subsection{6DOF dataset}
The ``6DOF dataset" is created with the constraint to maintain the end
effector of a 6-DOF robot arm pointed down (i.e., keep the orientation constant). The
data matrix is of size $21153$ by $6$. 

\subsection{Tilt dataset}
The Tilt dataset, like Nav, is an inequality constraint. Here, we model the scenario where a robot arm must keep its orientation within an allowable deviation from pointing straight down. The data matrix is of size $2000$ by $6$. 

\subsection{Handover dataset}
The Handover dataset is the most complex task we model in this work. It includes two robots, one mobile and one arm. The arm end effector must meet the top of the mobile robot in the workspace, allowing the arm to hand an object over to the other for transport. The data matrix is of size $2002$ by $8$. 

\end{comment}

==> RSS2020_TAMP Workshop_SMP_Learning/discussion.tex <==
\section{Discussion and Future Work}
\label{sec:discussion}
%
In this paper, we presented ways of learning constraint manifolds for sequential manifold planning. One of them is the novel {\ecmnnlong} ({\ecmnn}). {\ecmnn} is a method for learning representation for implicit functions, with an emphasis on representing equality constraints, while VAEs can also learn inequality constraints. We showed that {\ecmnn} has successfully learned equality constraint manifolds and that these manifolds can be used in a sequential motion planning method.

There are several interesting improvements and future directions to pursue.
First, there are still limitations with the current approach; in particular, our approach does not address the sign/polarity assignments of the implicit function value output, which we plan to address.
Second, we plan to do more comprehensive testing on higher-dimensional manifolds, and incorporate multiple learned constraints into a single motion plan with more subtasks. Further, we also plan to integrate manifolds learned with VAE into motion planning algorithms.


==> RSS2020_TAMP Workshop_SMP_Learning/ecmnn.tex <==
% \subsection{{\ecmnnlong} (\ecmnn)}
% \label{ssec:ecmnn}
%
% intro and motivation of why ECMNN can be useful:
We propose a novel neural network structure -- called \emph{\ecmnnlong} (\ecmnn) -- to become a learning representation that takes $\jointposition$ as input and outputs the prediction of the implicit function $\constraintfunction(\jointposition)$.
Moreover, we would like to train {\ecmnn} in a supervised manner, from demonstrations. One of the challenges is that the supervised training dataset is collected \emph{only} from demonstrations of data points which are on the equality constraint manifold $\onconstraintconfigspace$, called the \emph{on-manifold} dataset.
% and potentially corrupted with some noise. 
This is a reasonable assumption, since collecting both the on-manifold $\onconstraintconfigspace$ and off-manifold $\offconstraintconfigspace = \{ \jointposition \in \configspace \mid \constraintfunction(\jointposition) \neq \vct{0} \}$ datasets for supervised training will be tedious because the implicit function $\constraintfunction$ values of points in $\offconstraintconfigspace$ are typically unknown and hard to label.
We will show that even though our approach is only provided with data on $\onconstraintconfigspace$, it can still learn a useful representation of the manifold, sufficient for use in the SMP framework.

% I am not sure how to say this... Is this local neighborhood called a chart in Differential Geometry? Maybe Ragesh can help a bit?
Our goal is to learn a single global representation of the constraint manifold in form of a neural network. 
% However, according to Differential Geometry \citep{Lee00_IntroToSmoothManifolds}, each local neighborhood on the manifold contains important information. Moreover, collectively all these local neighborhoods characterize the global representation of the manifold. 
A manifold can be defined as a collection of local neighborhoods 
% called \emph{charts}
which resemble Euclidean spaces (\citet{Lee00_IntroToSmoothManifolds}). Therefore, a global representation of the manifold can be developed by constructing characterizations for its Euclidean-like local neighborhoods.

Our approach leverages local information on the manifold in the form of the tangent and normal spaces (\citet{Deutsch2015_TensorVotingGraph, GStrangIntroLinearAlgebra}).
% For a point on the manifold, the tangent and normal spaces are valid only for a small neighborhood surrounding the point. 
% With regard to the implicit function $\constraintfunction$, the tangent space is a vector space from which a vector can be chosen such that following this vector will keep the valuation of the function $\constraintfunction$ unchanged.  \imr{only locally/infintesimally, right? the value will change far from the point where it is tangent} 
% On the other hand, the normal space is a vector space from which a vector can be chosen such that following this vector will result in the maximum change in the valuation of the function $\constraintfunction$. \rag{I think previous two sentences are not required}
With regard to $\constraintfunction$, the tangent and normal spaces are equivalent to the null and row space,
% \rag{i think this should be row space or coimage space} 
respectively, of the matrix 
% $\constraintmanifoldjacobian = \frac{\partial \constraintfunction}{\partial \jointposition}$ 
$\constraintmanifoldjacobian = \left. \frac{\partial \constraintfunction({\jointposition})}{\partial {\jointposition}}\right|_{{\jointposition} = \Bar{\jointposition}}$, 
% evaluated at a point $\jointposition$ 
% \rag{$\Bar{\jointposition} = \jointposition$}, 
and valid in a small neighborhood around the point $\Bar{\jointposition}$.

Using on-manifold data, the local information of the manifold can be analyzed using Local Principal Component Analysis (Local PCA) (\citet{Kambhatla_LocalPCA}). Essentially, for each data point $\jointposition$ in the on-manifold dataset, we establish a local neighborhood using $\numnearestneighbor$-nearest neighbors ($\numnearestneighbor$NN) $\origKNN = \{\nearestneighborjointposition_1, \nearestneighborjointposition_2, \dots \nearestneighborjointposition_\numnearestneighbor\}$, with $\numnearestneighbor \geq \dimambient$. 
After a change of coordinates, $\jointposition$ becomes the origin of a new local coordinate frame $\lpcacoordframe$, and the $\numnearestneighbor$NN becomes $\recenteredKNN = \{\recenterednearestneighborjointposition_1, \recenterednearestneighborjointposition_2, \dots \recenterednearestneighborjointposition_\numnearestneighbor\}$ with $\recenterednearestneighborjointposition_\idxnearestneighbor = \nearestneighborjointposition_\idxnearestneighbor - \jointposition$ for all values of $\idxnearestneighbor$. Defining the matrix 
$\designmatrix = 
\begin{bmatrix} 
\recenterednearestneighborjointposition_1 & \recenterednearestneighborjointposition_2 & \hdots & \recenterednearestneighborjointposition_\numnearestneighbor \\
\end{bmatrix}\T \in \Re^{\numnearestneighbor \times \dimambient}
$, we can compute the covariance matrix $\samplecovariancematrix = \frac{1}{\numnearestneighbor-1} \designmatrix\T \designmatrix \in \Re^{\dimambient \times \dimambient}$.
The eigendecomposition of $\samplecovariancematrix = \covrighteigmat \covdiagsingularvalues \covrighteigmat\T$ gives us the Local PCA. 
The matrix $\covrighteigmat$ contains the eigenvectors of $\samplecovariancematrix$ as its columns in decreasing order w.r.t.\ the corresponding eigenvalues in the diagonal matrix $\covdiagsingularvalues$. These eigenvectors form the basis of $\lpcacoordframe$.

This local coordinate frame $\lpcacoordframe$ is tightly related to the tangent and normal spaces of the manifold at $\jointposition$. That is, the $(\dimambient - \dimconstraint)$ eigenvectors corresponding to the $(\dimambient - \dimconstraint)$ biggest eigenvalues of $\covdiagsingularvalues$ form a basis of the tangent space, while the remaining $\dimconstraint$ eigenvectors form the basis of the normal space. 
Furthermore, due to the characteristics of the manifold from which the dataset was collected, the $\dimconstraint$ smallest eigenvalues of $\covdiagsingularvalues$ will be close to zero, resulting in the $\dimconstraint$ eigenvectors associated with them forming the basis of the null space of $\samplecovariancematrix$. On the other hand, the remaining $(\dimambient - \dimconstraint)$ eigenvectors form the basis of the row space of $\samplecovariancematrix$. 
% Thus at $\jointposition$, the tangent space is equivalent to both the null space of $\constraintmanifoldjacobian$ and the row space of $\samplecovariancematrix$, while the normal space is equivalent to the row space of $\constraintmanifoldjacobian$ and the null space of $\samplecovariancematrix$.

To this end, we present several methods to define and train \ecmnn, as follows:
% \subsubsection{Determination of the Number of Constraints}
% ~\\
% We follow the same technique in \citep{Deutsch2015_TensorVotingGraph} for automatically determining the number of constraints $\dimconstraint$ from data, which is also the number of outputs of {\ecmnn}\footnote{Here we assume that the intrinsic dimensionality of the manifold at each point remains constant.}. Suppose the eigenvalues of $\samplecovariancematrix$ is $\{\covsingularvalue_1, \covsingularvalue_2, \dots, \covsingularvalue_\dimambient\}$ (in a decreasing order w.r.t. magnitude), then the number of constraint can be determined as $\dimconstraint = \argmax{\left(\left[\coveigval_1 - \coveigval_2, \coveigval_2 - \coveigval_3, \dots, \coveigval_{\dimambient-1} - \coveigval_{\dimambient}
% \right]\right)}$.

\subsection{Local Tangent and Normal Spaces Alignment}
% ~\\
% Previously Local Tangent Space Alignment (LTSA) \citep{Zhang02_LTSA} is a well-known manifold learning technique for embedding high-dimensional data into low-dimensional data, which is done by aligning the tangent space of each local neighborhood one another across the manifold. On the other hand, our method does not aim to achieve a low-dimensional embedding. Instead we try to learn the high-dimensional constraint manifold representation of the data for later use in motion planning.
% To-Do: explain why learning the the high-dimensional manifold representation?
% Our approach aims to align the following:
{\ecmnn} aims to align the following:
\begin{enumerate}[(a)]
    \item the null space of $\constraintmanifoldjacobian$ and the row space of $\samplecovariancematrix$, which both must be equivalent to the tangent space, and
    \item the row space of $\constraintmanifoldjacobian$ and the null space of $\samplecovariancematrix$, which both must be equivalent to the normal space
\end{enumerate}
for each local neighborhood of each point $\jointposition$ in the on-manifold dataset. 
Suppose the eigenvectors of $\samplecovariancematrix$ are $\{\coveigvec_1, \coveigvec_2, \dots, \coveigvec_\dimambient\}$ and the singular vectors of $\constraintmanifoldjacobian$ are $\{\constrjaceigvec_1, \constrjaceigvec_2, \dots, \constrjaceigvec_\dimambient\}$, where the indices indicate the decreasing order w.r.t. the eigenvalue/singular value magnitude. The null spaces of $\samplecovariancematrix$ and $\constraintmanifoldjacobian$ are spanned by $\{\coveigvec_{\dimambient-\dimconstraint+1}, \dots, \coveigvec_\dimambient\}$ and $\{\constrjaceigvec_{\dimconstraint+1}, \dots, \constrjaceigvec_\dimambient\}$, respectively. The two conditions above imply that the projection of the null space eigenvectors of $\constraintmanifoldjacobian$ into the null space of $\samplecovariancematrix$ should be $\vct{0}$, and similarly for the row spaces. 
% Similarly, the projection of the null space eigenvectors of $\samplecovariancematrix$ into the null space of $\constraintmanifoldjacobian$ shall be $\vct{0}$. 
Hence, we achieve this by training {\ecmnn} to minimize projection errors $\norm{\covnullspaceeigmat \covnullspaceeigmat\T \constrjacnullspaceeigmat}_2^2$ and $\norm{ \constrjacnullspaceeigmat \constrjacnullspaceeigmat\T \covnullspaceeigmat}_2^2$ with 
$\covnullspaceeigmat = 
\begin{bmatrix}
    \coveigvec_{\dimambient-\dimconstraint+1} & \dots & \coveigvec_\dimambient
\end{bmatrix}$
and 
$\constrjacnullspaceeigmat =  
\begin{bmatrix}
    \constrjaceigvec_{\dimconstraint+1} & \dots & \constrjaceigvec_\dimambient
\end{bmatrix}$.
%
% To-Do: also point out that the eigenvectors of Local PCA does NOT encode orientation, since sample covariance matrix is positive semi-definite, and hence the SVD has the left and right eigenvectors being the same --flipping the polarity of one of the eigenvectors will still lead to the same sample covariance matrix (SVD eigenvector v and -v is the same thing)--. On the other hand, the eigen decomposition of the Jacobian matrix results in eigenvectors who has polarity information, i.e. with eigenvalue fixed and positive, the eigenvector v and -v is NOT the same.
% To-Do: also point out that SVD result (in terms of eigenvectors ordering) for Local PCA is sensitive to the K-nearest-neighbors involved. For example on the case of 3D line constraint, the dimensionality of the constraints is 2, and neither of the eigenvectors in the normal space are dominant; however, a slight bit of noise in the data involved nearby point q1 and q2 (both on the manifold, and q1 != q2), can lead to two different eigenvector decompositions by SVD at q1 and q2. Hence, we cannot align each individual eigenvector of Local PCA with an eigenvector of the Jacobian J, as they may not correspond one another; what we can do is to align the null space of the Local PCA with the row space of the Jacobian, and to align the row space of the Jacobian with the null space of Local PCA, e.g. using projection error minimization.

\subsection{Data Augmentation with Off-Manifold Data}
% ~\\
The training dataset is on-manifold, i.e., each point $\jointposition$ in the dataset satisfies $\constraintfunction(\jointposition) = \vct{0}$. 
Through Local PCA on each of these points, we know the data-driven approximation of the normal space of the manifold at $\jointposition$. 
Hence, we know the directions where the violation of the equality constraint increases, i.e., the same or opposite direction of any vector from the approximate normal space. 
Since our future use of the learned constraint manifold on motion planning does not require the acquisition of the near-ground-truth value of $\constraintfunction(\jointposition) \neq \vct{0}$, we can set this off-manifold valuation of $\constraintfunction$ arbitrarily, as long as it does not interfere with the utility for projecting an off-manifold point onto the manifold. 
Therefore, we can augment our dataset with additional off-manifold data to achieve a more robust learning of {\ecmnn}. 
For each point $\jointposition$ in the on-manifold dataset, and for each eigenvector $\coveigvec$ that forms the basis of the normal space at $\jointposition$, we can add an off-manifold point $\augjointposition = \jointposition + \augidx \augmagnitude \coveigvec$ with a non-zero signed integer $\augidx$ and 
% a small positive scalar $\augmagnitude$ proportional to the square root of the biggest eigenvalue of $\samplecovariancematrix$. 
a small positive scalar $\augmagnitude$.
For such an augmented data point $\augjointposition$, we set the label satisfying $\norm{\constraintfunction(\augjointposition)}_2 = \abs{\augidx} \augmagnitude$. During training, we minimize the prediction error $\norm{(\norm{\constraintfunction(\augjointposition)}_2 - \abs{\augidx} \augmagnitude)}_2^2$ for each augmented point $\augjointposition$.

% To-Do: explain that {\ecmnn} is a generalization of the Signed Distance Function (SDF) Neural Network, up to a scale.

% To-Do: write a pseudo-algorithm describing our approach.


==> RSS2020_TAMP Workshop_SMP_Learning/experiments.tex <==
\section{Experiments}
\label{sec:experiments}
We compare the proposed {\ecmnn} method to a Variational Autoencoder (VAE), which is a popular method for learning a generative
model of a set of data (\citet{chen2016dynamic, kingma2013AutoEncodingVB, park2018multimodal}). Importantly, because
they embed data points as a distribution in the latent space, new latent vectors
can be sampled and decoded into unseen examples which fit the distribution of
the training data. VAEs make use of two neural networks in a neural autoencoder
structure during training, and they only use the decoder during generation. The
key idea that makes VAEs computationally tractable is that the distribution in
the latent space is assumed to be Gaussian. The loss function is a combination of the reconstruction error of the input and the KL divergence of the latent space distribution, weighted by a parameter $\beta$. 

We use the following network structures and parameters: 
For the Nav dataset, the VAE has two hidden layers with 6 and 4 units. The input size is 2 and the embedding size is 2. 
For the Plane dataset, the VAE has three hidden layers with 12, 9, and 6 units. The input size is 3 and the embedding size is 2.
For the Sphere, Orient, Tilt, and Handover datasets, the VAEs have the same structure: Four hidden layers with 8, 6, 6, and 4 units. The input sizes to the networks are 3, 6, 6, and 8, and the embedding sizes are 2, 5, 3, and 7, respectively.
All VAE models have $\beta$ = 0.25 and use batch normalization. We train for 500 epochs for Handover, and 200 otherwise.

% 1. compare h values
\subsection{Evaluate Implicit Functions on Datasets}
\label{sec:experiment1}
We compare the performance of the models using the implicit function value $\constraintfunction$. In the case of the VAE models, we take the reprojected data $\hat{X}$ and evaluate each configuration with $\constraintfunction$. In the case of the \ecmnn, the output of the network is the estimated implicit function value of the input, so we can directly use it. We report the mean and standard deviation of $\constraintfunction$ for each dataset in Table \ref{table:experiment1}. Note that for Nav and Tilt datasets, $h_M$ does not need to be 0 for a configuration to be valid, since these are inequality constraints. Values less than 1 for Nav and less than 0.1 for Tilt adhere to the constraints.

% gsutanto: please feel free to remove this figure/sub-experiment, if you have a more interesting figure
% \subsubsection{Level Set Contour Plot and the Normal Space Vector Field of Learned {\ecmnn}}
%
In Fig.~\ref{sfig:levelset_contour_and_jac_vector_field}, we plot the level set contour as well as the normal space eigenvector field of an {\ecmnn} after training on a 3D unit sphere constraint dataset. We see that at both cross-sections $y=0$ (left) and $z=0$ (right), the contours are close to circular, which is expected for a unit sphere constraint manifold.
%

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.66\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{figures/contourplot_ltsann_epoch_25.png}
        \vspace{-0.8cm}
        \caption{Level set contour plot and the learned {\ecmnn}'s normal space eigenvector field, after training on a 3D unit sphere constraint dataset.}
        \label{sfig:levelset_contour_and_jac_vector_field}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{figures/hourglass_learned.png}
        \caption{Visualization of a planned path on a learned manifold (sphere).}
        \label{sfig:hourglass_learned}
    \end{subfigure}
\end{figure}

% 2. compare generated points on the manifold
\subsection{Evaluate Implicit Functions on Generated Configurations}
\label{sec:experiment2}
We use the trained VAE models from Sec. \ref{sec:experiment1} to generate 100,000 new, on-manifold configurations for each constraint. We then evaluate these configurations with the implicit function $h_M$ and report the mean and standard deviation in Table \ref{table:experiment2}.

% 3. compare plans produced by SMP with these methods incorporated 
\subsection{Sequential Motion Planning on Learned Manifolds}
\label{sec:experiment3}
In this experiment, we incorporate a learned manifold into the planning framework developed and introduced in \citet{englert2020sampling}. The Sphere dataset (see Section \ref{sec:datasets}) is used to learn a manifold representation with {\ecmnn}. This learned manifold is combined with two analytical manifolds representing paraboloids. A motion planning problem is defined on these three manifolds where a 3D point has to find a path from a start configuration on one of the paraboloids to a goal configuration on the other. See Figure \ref{sfig:hourglass_learned} for a visualization of the manifolds and a found path with SMP.

\begin{table}
  \caption{Experiment A -- $\constraintfunction$ on Datasets.}
  \label{table:experiment1}
  \centering
  \resizebox{\columnwidth}{!}{%
  \begin{tabular}{ccc|cc|cc|cc|cc|cc}
    \toprule
         Method & \multicolumn{12}{c}{Dataset} \\
     & \multicolumn{2}{c}{Nav} & \multicolumn{2}{c}{Sphere} & \multicolumn{2}{c}{Plane} & \multicolumn{2}{c}{Orient} & \multicolumn{2}{c}{Tilt} & \multicolumn{2}{c}{Handover} \\
     \midrule
              & $\mu$ & $\sigma$ & $\mu$ & $\sigma$ & $\mu$ & $\sigma$ & $\mu$ & $\sigma$ & $\mu$ & $\sigma$ & $\mu$ & $\sigma$ \\
    \midrule
      VAE     & 0.42 & 0.18 & 0.08 & 0.03 & 0.16 & 0.12 & 0.01 & 0.03 & 0.09 & 0.07 & 0.56 & 0.47 \\
    %   \ecmnn     & N/A & N/A & 0.0417 & 0.0583 & 0.45648336 & 1.3869419 & -0.048004348 & 0.9334844 & N/A & N/A & 0.23925124 & 0.7597604 \\
      \ecmnn     & N/A & N/A & 0.04 & 0.06 & 0.46 & 1.39 & -0.05 & 0.93 & N/A & N/A & 0.24 & 0.76 \\
    \bottomrule
  \end{tabular}
  }
\end{table}

\begin{table}
    \caption{Experiment B -- $\constraintfunction$ on Generated Configurations.}
  \label{table:experiment2}
  \centering
  \resizebox{\columnwidth}{!}{%
  \begin{tabular}{ccc|cc|cc|cc|cc|cc}
    \toprule
         Method & \multicolumn{12}{c}{Dataset} \\
     & \multicolumn{2}{c}{Nav} & \multicolumn{2}{c}{Sphere} & \multicolumn{2}{c}{Plane} & \multicolumn{2}{c}{Orient} & \multicolumn{2}{c}{Tilt} & \multicolumn{2}{c}{Handover} \\
     \midrule
              & $\mu$ & $\sigma$ & $\mu$ & $\sigma$ & $\mu$ & $\sigma$ & $\mu$ & $\sigma$ & $\mu$ & $\sigma$ & $\mu$ & $\sigma$ \\
    \midrule
      VAE     & 0.58 & 0.18 & 0.10 & 0.03 & 0.14 & 0.08 & 0.01 & 0.01 & 0.96 & 0.30 & 0.10 & 0.02 \\
    \bottomrule
  \end{tabular}
  }
\end{table}

% \begin{table}
%     \caption{Experiment C -- Motion plans.}   
%   \label{table:experiment3}
%   \centering
%   \resizebox{\columnwidth}{!}{%
%   \begin{tabular}{ccc|cc|cc|cc|cc|cc}
%     \toprule
%          Method & \multicolumn{12}{c}{Dataset} \\
%      & \multicolumn{2}{c}{Nav} & \multicolumn{2}{c}{Sphere} & \multicolumn{2}{c}{3DOF} & \multicolumn{2}{c}{6DOF} & \multicolumn{2}{c}{Tilt} & \multicolumn{2}{c}{Handover} \\
%      \midrule
%               & $\mu$ & $\sigma$ & $\mu$ & $\sigma$ & $\mu$ & $\sigma$ & $\mu$ & $\sigma$ & $\mu$ & $\sigma$ & $\mu$ & $\sigma$ \\
%     \midrule
%       VAE     &  &  &  &  &
%                  &  &  &  &
%                 &  &  & \\
%       \ecmnn     &  &  &  &  &
%                  &  &  &  &
%                 &  &  & \\
%     \bottomrule
%   \end{tabular}
%   }
% \end{table}


==> RSS2020_TAMP Workshop_SMP_Learning/introduction.tex <==
\section{Introduction}
\label{sec:introduction}

% introduce topic of sequential motion planning in TAMP 
Many practical robotic applications require planning robot motions with constraints, such as maintaining an orientation or reaching a particular location. Planning becomes more complicated when the  task consists of many subtasks that must be completed in sequence. In this case, task and motion planning frameworks \cite{kaelbling2013integrated, dantam2016incremental, konidaris2018skills, toussaint2018differentiable, dantam2018task, barry2013hierarchical, cambon2009hybrid} can be used to handle long planning horizons and a wide range of tasks. 
% motivation: some constraints are hard to describe; some maybe hard to sample from; we show this for a wide variety of constraint types; give pouring example
However, some constraints may be difficult to describe analytically, or it may be difficult to sample constraints that adhere to them. For example, if the task is to pour a liquid from a bottle into a cup, it is not immediately clear how to encode the motion constraints for a planning algorithm.

% describe our work at a high level
In this work, we focus on learning constraint manifolds for use in constrained motion planning algorithms \cite{englert2020sampling, stilman2010global, berenson2011task, jaillet2013asymptotically, kim2016tangent, kingston2019ijrr, csucan2012motion, cortes2004sampling}.
To this end, we investigate two different approaches: Variational autoencoders (VAE) following \citet{kingma2013AutoEncodingVB}, and {\ecmnnlong}  (\ecmnn), a method we propose which learns the implicit function value of equality constraints. We evaluate these techniques on six datasets of varying size and complexity, and we present preliminary resulting motion plans.

\begin{comment}
% This work builds on previous developments in constrained SBMP for sequential
% tasks. A new framework for constrained sequential motion planning formulates the
% problem as a constrained optimization problem, and each subtask is solved in
% sequence. The algorithm uses dynamic programming over task switching points, or
% ``intersection points", to minimize the cost of the solution path while keeping
% computation cost low. 

% With this approach, constraints are described as manifolds in configuration
% space defined by equality constraints. Here, we intend to expand the approach to
% incorporate learned constraints from data, 
% where the manifold constraint is not known analytically.

% TODO: check the list of techniques and the datasets, also indicate the novelty of {\ecmnn}?
To begin, we evaluate several manifold learning techniques on multiple datasets.
The techniques we discuss in this work are:
% Autoencoders (AE); 
Variational Autoencoders (VAE); 
% Feedforward Neural Networks (NN); 
% Singular Value Decomposition (SVD); 
% Isomap; 
and 
% Locally Linear Embedding (LLE).
{\ecmnnlong} ({\ecmnn}).
We evaluate these models on 6 datasets of varying size and complexity.

First we give a summary of the planning framework. Then, we discuss motivation
for learning manifolds from data, go over the techniques which are
considered, and briefly cover some related work. Next, we describe each dataset.
Then, we show results for each technique. Finally, we discuss how the learned
manifold constraints can be incorporated into a robotic motion planner, and we 
conclude with a summary of the findings and the next steps for this work. 
\end{comment}

==> RSS2020_TAMP Workshop_SMP_Learning/macros.tex <==
\newcommand{\argmax}[1]{\underset{#1}{\operatorname{arg}\operatorname{max}}\;}
\newcommand{\argmin}[1]{\underset{#1}{\operatorname{arg}\operatorname{min}}\;}
\renewcommand{\min}[1]{\underset{#1}{\operatorname{min}}\;}
\renewcommand{\max}[1]{\underset{#1}{\operatorname{max}}\;}
\newcommand{\st}{\t{s.t.}}

\newcommand{\etal}{\textit{et al}. }


\newcommand{\pe}[1]{{\color{blue} \textrm{PE: #1}}}
\newcommand{\gs}[1]{{\color{red} \textrm{GS: #1}}}
\newcommand{\imr}[1]{{\color{cyan} \textrm{IMR: #1}}}

\newcommand{\rag}[1]{{\color{magenta} \textrm{RKR: #1}}}
\newcommand{\new}[1]{{\color{blue} \textrm{#1}}}

\renewcommand{\v}{\boldsymbol}
\renewcommand{\t}[1]{{\textrm{#1}}}

\newcommand{\R}{\mathbb{R}}
\newcommand{\data}{\mathcal{D}}

\newcommand{\eq}{Equation~} 
\newcommand{\eqs}{Equations~}
\newcommand{\fig}{Figure~}
\newcommand{\alg}{Algorithm~}
\newcommand{\algs}{Algorithms~}
\newcommand{\sect}{Section~}
\newcommand{\cha}{Chapter~}
\newcommand{\tab}{Table~}

\newcommand{\opt}{^\star}

\ifdefined\T
\renewcommand{\T}{^\top}
\else
\newcommand{\T}{^\top}
\fi

\newcommand{\mat}[3][.9]{
  \renewcommand{\arraystretch}{#1}{\scriptscriptstyle{\left(
    \hspace*{-1ex}\begin{array}{#2}#3\end{array}\hspace*{-1ex}
  \right)}}\renewcommand{\arraystretch}{1.2}
}

\newcommand{\bmat}[3][.9]{
  \renewcommand{\arraystretch}{#1}{\scriptscriptstyle{\left[
    \hspace*{-1ex}\begin{array}{#2}#3\end{array}\hspace*{-1ex}
  \right]}}\renewcommand{\arraystretch}{1.2}
}

\newcommand{\inv}{^{-1}}
\newcommand{\diag}{\text{diag}}

\newcommand{\comma}{~,}
\newcommand{\period}{~.}

\newcommand{\ga}{\alpha}
\newcommand{\gb}{\beta}
\newcommand{\gd}{\delta}
\newcommand{\gD}{\Delta}
\renewcommand{\ge}{\epsilon}
\renewcommand{\gg}{\gamma}
\newcommand{\gG}{\Gamma}
\newcommand{\gl}{\lambda}
\newcommand{\gL}{\Lambda}
\newcommand{\gm}{\mu}
\newcommand{\gn}{\nu}
\newcommand{\gN}{\nabla}
\newcommand{\gk}{\kappa}
\newcommand{\go}{\omega}
\newcommand{\gO}{\Omega}
\newcommand{\gp}{\phi}
\newcommand{\gph}{\varphi}
\newcommand{\gP}{\Phi}
\newcommand{\gr}{\rho}
\newcommand{\grh}{\varrho}
\newcommand{\gsi}{\sigma}
\newcommand{\gSi}{\Sigma}
\newcommand{\gt}{\theta}
\newcommand{\gT}{\Theta}
\newcommand{\gv}{\vartheta}
\newcommand{\gx}{\xi}
\newcommand{\gX}{\Xi}
\newcommand{\gY}{\Upsilon}
\newcommand{\gz}{\zeta}

% math environments
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{theorem}{Theorem}

\newcommand{\lemmaautorefname}{Lemma}
\newcommand{\algorithmautorefname}{Algorithm}

==> RSS2020_TAMP Workshop_SMP_Learning/manifold_learning.tex <==
\section{Manifold Learning}
\label{sec:manifold_learning}
Learning constraint manifolds from data is attractive for multiple reasons. 
For example, it may be easier for a human to demonstrate a task rather than specifying constraints analytically,
% we may want to encode constraints that are not strict equalities, 
or we may want to reduce the amount of expert information needed. 

% To this end, we investigate several existing techniques for manifold learning to
% use within our framework. 
\begin{comment}
\subsection{Problem Statement}
Our goal here is to focus on a single manifold as opposed to the entire sequence. We
do not assume the analytical description of the manifold (e.g., $h_M$) is known.
Rather, we have a set of data $x \in \mathbb{R}^d$. These $n$ datapoints are
configurations in $\mathbb{R}^n$ which adhere to the constraint $M$. That is, $x_i \in C_M \forall x_i \in
X$. We seek a model $A_\theta$, learned using our dataset $X$, which encodes an approximate representation $\hat{M}$ of the manifold constraint in a lower-dimensional space in
$\mathbb{R}^{\hat{d}}, \hat{d} \leq d$. 

For the purposes of planning, we are mainly interested in the capability of the learned model to reconstruct
the data accurately. In particular, we would like $\hat{M}$ learned by
$A_\theta$ to be able to transform data points between the original (ambient)
space in $\mathbb{R}^d$ and the learned embedding space in
$\mathbb{R}^{\hat{d}}$. 
To achieve this, we use the mean squared error (MSE) of $\hat{x}$ and $x$ as a
metric, which we call the ``reprojection error" and would like to minimize: 
$$ MSE = \frac{1}{n} \sum_{i}^n (\hat{x}_i - x_i)^2 $$
A low MSE indicates that the learned latent embedding of the manifold estimates
the dataset well, and therefore it is an accurate representation of the manifold
constraint. 

Additionally, we consider the ``?'' metric. Given a point $X$ which originally was on the manifold (i.e., $h(x) = 0$) and its reprojected image $\hat{x}$, we define the metric %TODO fill this name in
as $h(\hat{x})$. This value should ideally also be $0$, indicating that even if the point is not exactly reconstructed as before, it is still a valid configuration for the given constraint.

Because constraints will often be in a lower dimension than the ambient configuration space, this motivates the use of dimensionality reduction techniques on data. 
In general, the constraint manifolds may have arbitrary structure; we assume they
have been sampled sufficiently densely but otherwise make no further
assumptions.  % TODO is this true?

% \subsection{Autoencoders}

\subsection{Variational Autoencoders}
Variational Autoencoders (VAEs) are a popular method for learning a generative
model of a set of data (\citep{chen2016dynamic, kingma2013AutoEncodingVB, habibie2017recurrent, park2018multimodal}). Importantly, because
they embed data points as a distribution in the latent space, new latent vectors
can be sampled and decoded into unseen examples which fit the distribution of
the training data. VAEs make use of two neural networks in a neural autoencoder
structure during training, and they only use the decoder during generation. The
key idea that makes VAEs computationally tractable is that the distribution in
the latent space is assumed to be Gaussian. 
\end{comment}

\begin{comment}
\subsection{Singular Value Decomposition}
Principal Component Analysis (PCA) (\citet{tipping1999probabilistic}) and
Singular Value Decomposition (SVD) (\citet{halko2011finding}) are used for linear
dimensionality reduction. PCA is a method whose goal, given a set of $n$ data points $X \in
\mathbb{R}^d$, is to find a set of $k < d$ orthogonal vectors which explain the
most variance in the dataset. Several techniques can be used to find these
orthogonal vectors (also known as principal axes); SVD is one of them.
In essence, SVD decomposes an $n$ by $d$ data matrix $A$ into the diagonal form 
$A = USV^T$
where $S$ is a diagonal matrix that contains the singular values $\sigma_i$ (the
square roots of the eigenvalues) of $A$, and $U$ and $V$ are composed of the
eigenvectors of $AA^T$ and $A^TA$, respectively. With $\sigma$ in decreasing
order, the first $k$ columns of $V$ ($V_k$) can be used as the principal axes
for the data (see \citet{shlens2014tutorial} for a more in-depth explanation).
The data $X$ can be transformed into the new $k$-dimensional space  via
projection: $Y = XV_k$
and, unlike LLE, transformed data can be reprojected easily with $V_k^T$ since
$V_k$ is an orthonormal matrix: $\hat{X} = YV_k^T$.

\subsection{Locally Linear Embedding}

% this is pretty long. we might shorten it to something like this:
Locally Linear Embedding (LLE) produces a global embedding based on local structure. The idea is to first use a set of $k$ nearest neighbors of each point to linearly reconstruct a point $\vec{X}_i$ as close to its true value as possible.
Secondly, using these linear reconstruction weights $W_{ij}$, LLE computes
lower-dimensional embedding vectors of each point, which are computed such that they minimize the difference between the embedding and a linear reconstruction of the embeddings of its nearest neighbors using the same $W_{ij}$. Thus, LLE assumes that local structure is preserved in the learned embedding.

One of the main drawbacks of LLE for our work is
that it does not encode a method for reprojecting embeddings into the ambient space. Additionally, if the
manifold is tightly folded (imagine a tightly wound spring), points on a loop
above or below $\vec{X}_i$ may be chosen as nearest neighbors when in reality the
geodesic distance between them may be quite large. 
%%%%

% Locally Linear Embedding (LLE) has several variants (\citet{roweis2000nonlinear},
% \citet{zhang2007mlle}, \citet{donoho2003hessian}, \citet{zhang2002principal}).
% LLE produces a global embedding based on local structure. The idea is to use a
% small set $K_i$ of $k$ nearest neighbors of each point $\vec{X}_i \in
% \mathbb{R}^d$ to linearly reconstruct $\vec{X}_i$ as close to its true value as
% possible.
% % $$ \min_{W_{ij}} |\vec{X}_i - \sum_{j \in \kappa_i} (W_{ij}\vec{X}_j ) |^2 $$
% Then, using these linear reconstruction weights $W_{ij}$, LLE computes the
% lower-dimensional embedding vectors $\vec{Y}_i \in \mathbb{R}^{\hat{d}}$
% ($\hat{d} \leq d$) of each point. The vectors $\vec{Y}_i$ are computed such that
% they minimize the embedding cost function
% $$ \min_{Y_i} \hspace{0.5em} \Phi (Y) = \sum_i | \vec{Y}_i - \sum_{j \in K_i}( W_{ij}\vec{Y}_{j} ) | ^2$$
% where the weights $W_{ij}$ are fixed (from the first reconstruction step in
% $\mathbb{R}^d$), and the $\vec{Y}_i$ (the embedding of point $\vec{X}_i$) are
% the optimization variables. 

% LLE operates under the assumption that local neighborhoods structure in the
% original space should be similar to the local structure in the embedding space,
% and hence the $W_{ij}$ are preserved. Thus, this is a method that produces a
% neighborhood-preserving mapping to a lower-dimensional embedding. 

% One of the main drawbacks of LLE for the problems described in this paper is
% that it does not encode a method for reprojecting data from
% $\mathbb{R}^{\hat{d}}$ back into $\mathbb{R}^d$. Additionally, care must be
% taken with the metric used to determine nearest neighbors of $\vec{X}_i$. If the
% manifold is tightly folded (imagine a tightly wound spring), points on a loop
% above or below $\vec{X}_i$ may be chosen for $K_i$ when in reality the
% geodesic distance between them may be quite large. 

\subsection{Isomap}
Isomap, named for isometric mapping, is a manifold learning technique that
approximates geodesic distances via a graph constructed from the data $X$
(\citet{tenenbaum2000global}). Similarly to LLE, each point $\vec{X}_i$ has a
nearest neighborhood $K_i$ of size $k$. However, this neighborhood is not
used to reconstruct $\vec{X}_i$. Rather, a graph is constructed
where the vertices $V$ represent the data points in $X$, and the edges $E$
connect points in a neighborhood. Then, finding the
shortest path between two nodes using an algorithm such as Dijkstra's is
equivalent to approximating the geodesic distance on the manifold between two
data points. After computing all pairwise distances, the final step to produce
an embedding is to apply Multidimensional Scaling (MDS, \citet{borg2005modern},
\citet{kruskal1978multidimensional}) to $D$. MDS uses eigenvalue decomposition
given a distance or dissimilarity matrix (here, $D$) to produce data $\hat{X}$
that preserve these distances. Like LLE, Isomap lacks the ability to transform
embedded data points back into the original space and may not
produce accurate results if the manifold is very crumpled or folded. 
\end{comment}

\input{ecmnn}


==> RSS2020_TAMP Workshop_SMP_Learning/preamble.tex <==
% our commands
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Package options
\usepackage{graphics} % for pdf, bitmapped graphics files
\usepackage{epsfig} % for postscript graphics files
%\usepackage{mathptmx} % assumes new font selection scheme installed
\usepackage{times} % assumes new font selection scheme installed
\usepackage{amsmath} % assumes amsmath package installed
\usepackage{amssymb}  % assumes amsmath package installed
\usepackage{caption}
\usepackage{subcaption}
% \captionsetup{compatibility=false}
% \usepackage[caption=false]{subfig}
\let\labelindent\relax
\usepackage[shortlabels]{enumitem}
\usepackage{multirow}
\usepackage{booktabs}
\usepackage[nocomma]{optidef}
\usepackage{cancel}
\usepackage{color}
\usepackage[normalem]{ulem}

\pdfminorversion=4

\newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}

\DeclarePairedDelimiter\abs{\lvert}{\rvert}%
\DeclarePairedDelimiter\norm{\lVert}{\rVert}%

% Swap the definition of \abs* and \norm*, so that \abs
% and \norm resizes the size of the brackets, and the 
% starred version does not.
\makeatletter
\let\oldabs\abs
\def\abs{\@ifstar{\oldabs}{\oldabs*}}
%
\let\oldnorm\norm
\def\norm{\@ifstar{\oldnorm}{\oldnorm*}}
\makeatother

\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}
% \newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\ecmnnlong}{Equality Constraint Manifold Neural Network}
\newcommand{\ecmnn}{ECoMaNN}
\newcommand{\configspace}{\mathcal{C}}
\newcommand{\dimambient}{d}
\newcommand{\dimconstraint}{l}
\newcommand{\deltat}{\Delta t}
\newcommand{\jacobian}{\mathbf{J}}
\newcommand{\jointposition}{\mathbf{q}}
\newcommand{\jointvelocity}{\dot{\mathbf{q}}}
\newcommand{\jointacceleration}{\ddot{\mathbf{q}}}
\newcommand{\cartesianposition}{\mathbf{x}}
\newcommand{\cartesianvelocity}{\dot{\mathbf{x}}}
\newcommand{\eye}{\mathbf{I}}
\newcommand{\numconstraintmanifold}{n}
\newcommand{\constraintmanifold}{M}
\newcommand{\constraintmanifoldsequence}{\mathcal{\constraintmanifold}}
\newcommand{\constraintfunction}{{h}_{\constraintmanifold}}
\newcommand{\constraintmanifoldjacobian}{\jacobian_\constraintmanifold}
\newcommand{\onconstraintconfigspace}{{\configspace}_{\constraintmanifold}}
\newcommand{\offconstraintconfigspace}{{\configspace}_{\cancel{\constraintmanifold}}}
\newcommand{\numnearestneighbor}{K}
\newcommand{\idxnearestneighbor}{k}
\newcommand{\KNNset}{\mathcal{K}}
\newcommand{\origKNN}{\hat{\KNNset}}
\newcommand{\recenteredKNN}{\tilde{\KNNset}}
\newcommand{\nearestneighborjointposition}{\hat{\jointposition}}
\newcommand{\recenterednearestneighborjointposition}{\tilde{\jointposition}}
\newcommand{\designmatrix}{\mathbf{X}}
\newcommand{\samplecovariancematrix}{\mathbf{S}}
\newcommand{\lefteigmat}{\mathbf{U}}
\newcommand{\diagsingularvalues}{\mathbf{\Sigma}}
\newcommand{\eigval}{\lambda}
\newcommand{\righteigmat}{\mathbf{V}}
% \newcommand{\covdiagsingularvalues}{\diagsingularvalues_{\samplecovariancematrix}}
% \newcommand{\covrighteigmat}{\righteigmat_{\samplecovariancematrix}}
\newcommand{\covdiagsingularvalues}{\diagsingularvalues}
\newcommand{\coveigval}{\eigval}
\newcommand{\covsingularvalue}{{\coveigval}^2}
\newcommand{\covrighteigmat}{\righteigmat}
\newcommand{\lpcacoordframe}{\mathcal{F}}
\newcommand{\coveigvec}{\vct{v}}
\newcommand{\constrjaceigvec}{\vct{e}}
\newcommand{\nullspaceid}{\text{N}}
\newcommand{\covnullspaceeigmat}{\righteigmat_{\nullspaceid}}
\newcommand{\constrjacrighteigmat}{\mathbf{E}}
\newcommand{\constrjacnullspaceeigmat}{\constrjacrighteigmat_{\nullspaceid}}
\newcommand{\augjointposition}{\check{\jointposition}}
\newcommand{\augidx}{i}
\newcommand{\augmagnitude}{\epsilon}
\newcommand{\cost}{J}
\newcommand{\tpath}{\tau}
\newcommand{\tpathset}{\vct{\tpath}}
\newcommand{\costfunctional}{\mathcal{\cost}}
\newcommand{\tpathspace}{\mathcal{T}}
\newcommand{\freeconfigspaceoperator}{\Upsilon}

% just some definitions to write our equations easier 

\newcommand{\argmin}{\operatorname*{arg\:min}}
\newcommand{\argmax}{\operatorname*{arg\:max}}

\newcommand{\mpg}[1]{{\color{MPG} #1}}    % highlight command 1
\newcommand{\gra}[1]{{\color{mgra} #1}}   % highlight command 1
\newcommand{\dre}[1]{{\color{dred} #1}}   % highlight command 1
\newcommand{\lre}[1]{{\color{lred} #1}}

%%%% highlight
\newcommand{\hl}[1]{\mpg{#1}}

%%% space
%\setlength{\parindent}{0cm}
% \setlength{\belowcaptionskip}{-3pt}
\newcommand{\qq}{\qquad}
\newcommand{\qqq}{\quad\qquad}
\newcommand{\qqqq}{\qquad\qquad}

%%% operators
\newcommand \dd[1]  { \,\textrm d{#1}                       }   % infintesimal
\newcommand \de[2]  { \frac{\mathrm d{#1}}{\mathrm d{#2}}   }   % first order
\newcommand{\Exp}{\mathbb{E}}
\newcommand{\Ent}{\mathbb{H}}
\newcommand{\Cov}{\operatorname{cov}}
\renewcommand{\H}{\mathcal{H}}
\newcommand{\KL}{\text{KL}}
\renewcommand{\Re}{\mathbb{R}}
\newcommand{\one}{\vec{1}\vec{1}\Trans}
\newcommand{\Dcal}{\mathcal{D}}
\newcommand{\N}{\mathcal{N}}
\renewcommand{\L}{\mathcal{L}}
\newcommand{\Trans}{^{\intercal}}
\newcommand{\rep}{\text{rep}}
\newcommand{\base}{\text{base}}
\newcommand{\eval}{\text{eval}}
\newcommand{\diag}{\operatorname{diag}}

%%% often used bold symbols (vectors, matrices)
%%%%%%%%%%%%%%%%%% gsutanto's (START) %%%%%%%%%%%%%%%%%%
\newcommand{\xd}{\dot{x}}
\newcommand{\xdd}{\ddot{x}}
%%%%%%%%%%%%%%%%%%% gsutanto's (END) %%%%%%%%%%%%%%%%%%%
% \newcommand{\vmu}{\boldsymbol{\mu}}
\newcommand{\vxi}{\boldsymbol{\xi}}
\newcommand{\vphi}{\boldsymbol{\phi}}
\newcommand{\vpsi}{\boldsymbol{\psi}}
\newcommand{\valpha}{\boldsymbol{\alpha}}
\newcommand{\vbeta}{\boldsymbol{\beta}}
% \newcommand{\vw}{\vec{w}}
\newcommand{\vct}[1]{\boldsymbol{#1}} % vector
\newcommand{\mat}[1]{\boldsymbol{#1}} % matrix
\newcommand{\vy}{\vec{y}}
\newcommand{\vx}{\vec{x}}
\newcommand{\vz}{\vec{z}}
\newcommand{\vf}{\vec{f}}
\newcommand{\vu}{\vec{u}}
\newcommand{\vk}{\vec{k}}
\newcommand{\vs}{\vec{s}}
\newcommand{\mX}{\boldsymbol{X}}
\newcommand{\mA}{\mathbf{A}}
\newcommand{\mB}{\mathbf{B}}
\newcommand{\mC}{\mathbf{C}}
\newcommand{\mQ}{\mathbf{Q}}
\newcommand{\mR}{\mathbf{R}}
\newcommand{\mV}{\mathbf{V}}
\newcommand{\mP}{\mathbf{P}}
\newcommand{\ms}{\mathbf{s}}
\newcommand{\mS}{\mathbf{S}}
\newcommand{\mK}{\mathbf{K}}
\newcommand{\mJ}{\mathbf{J}}
\newcommand{\mY}{\mathbf{Y}}
\newcommand{\mW}{\mathbf{W}}
\newcommand{\mZ}{\mathbf{Z}}
\newcommand{\mSigma}{\boldsymbol{\Sigma}}
\newcommand{\mGamma}{\boldsymbol{\Gamma}}
\newcommand{\mPhi}{\boldsymbol{\Phi}}

\newcommand{\sA}{\boldsymbol{\mathsf{A}}}
\newcommand{\sB}{\boldsymbol{\mathsf{B}}}
\newcommand{\sC}{\boldsymbol{\mathsf{C}}}

% transpose
\newcommand{\T}{^{\textrm T}} % transpose


\newcommand{\ga}{\alpha}
\newcommand{\gb}{\beta}
\newcommand{\gd}{\delta}
\newcommand{\gD}{\Delta}
\renewcommand{\ge}{\epsilon}
\renewcommand{\gg}{\gamma}
\newcommand{\gG}{\Gamma}
\newcommand{\gl}{\lambda}
\newcommand{\gL}{\Lambda}
\newcommand{\gm}{\mu}
\newcommand{\gn}{\nu}
\newcommand{\gN}{\nabla}
\newcommand{\gk}{\kappa}
\newcommand{\go}{\omega}
\newcommand{\gO}{\Omega}
\newcommand{\gp}{\phi}
\newcommand{\gph}{\varphi}
\newcommand{\gP}{\Phi}
\newcommand{\gr}{\rho}
\newcommand{\grh}{\varrho}
\newcommand{\gsi}{\sigma}
\newcommand{\gSi}{\Sigma}
\newcommand{\gt}{\theta}
\newcommand{\gT}{\Theta}
\newcommand{\gv}{\vartheta}
\newcommand{\gx}{\xi}
\newcommand{\gX}{\Xi}
\newcommand{\gY}{\Upsilon}
\newcommand{\gz}{\zeta}
\newcommand{\R}{\mathbb{R}}
\newcommand{\period}{~.}
\renewcommand{\t}[1]{{\textrm{#1}}}
\newcommand{\st}{\t{s.t.}}

% author comments
\newcommand{\pe}[1]{{\color{blue} \textrm{PE: #1}}}
\newcommand{\gs}[1]{{\color{red} \textrm{GS: #1}}}
\newcommand{\imr}[1]{{\color{cyan} \textrm{IMR: #1}}}

\newcommand{\rag}[1]{{\color{magenta} \textrm{RKR: #1}}}

==> RSS2020_TAMP Workshop_SMP_Learning/related_work.tex <==
\section{Related work}
\label{sec:related_work}
% TODO: move any related work to the intro, cut down on CSBMP and include more manifold learning. 

\subsection{Constrained SBMP} \label{csbmp} Sampling-based motion planning
(SBMP) is a broad field which tackles the problem of motion planning by using
randomized sampling techniques to build a tree or graph of configurations (also
called samples). The resulting tree or graph can then be used to plan paths
between configurations. This is in contrast to other motion planning techniques,
which may optimize an objective function over a continuous space of trajectories
(e.g., \citet{kalakrishnan2011stomp}) or use the gradient of a potential field
to guide a path toward a goal configuration (e.g., \citet{khatib1986real}).
Many SBMP algorithms derive from one of the following SBMP methods:
Rapidly-exploring random tree (RRT) (\citet{lavalle1998rapidly,
lavalle2006planning}), probabilistic roadmap (PRM)
(\citet{kavraki1994randomized}), and their optimal counterparts RRT* and PRM*
(\citet{karaman2011sampling}). These methods work by sampling the search space,
connecting samples if the edge between them does not collide with obstacles, and
then querying the tree or graph for a valid path that reaches the goal state. A
collision detector is generally assumed to exist, which reports whether or not a
state is in collision with obstacles in the environment. 

A more challenging and realistic motion planning task is that of constrained
SBMP, where there are motion constraints beyond simply obstacle avoidance.
Constraints will often lead to a free configuration space manifold $C_{free} \in
\mathbb{R}^{d'}$ of lower dimension than the ambient configuration space $C \in
\mathbb{R}^d$. (For example, consider the constraint where an arm must stay at a
particular height. A joint that moves the arm up and down will have an effective
space of only one value, and hence the rest of the configuration space is
"squashed" down a dimension.) Randomized sampling in a $d$-dimensional space
will produce samples on a $d' < d$ -dimensional space with probability 0, so
additional measures must be taken to produce valid samples for planning. Another
complication arises when there is not just one constraint, but many, which may
have a specific order in which they must be met in order to achieve the task
goal.

\subsection{Manifold Learning}

==> RSS2020_TAMP Workshop_SMP_Learning/use_in_planning.tex <==
\section{Use in planning}
\label{sec:use_in_planning}

==> macros.tex <==
\newcommand{\argmax}[1]{\underset{#1}{\operatorname{arg}\operatorname{max}}\;}
\newcommand{\argmin}[1]{\underset{#1}{\operatorname{arg}\operatorname{min}}\;}
\renewcommand{\min}[1]{\underset{#1}{\operatorname{min}}\;}
\renewcommand{\max}[1]{\underset{#1}{\operatorname{max}}\;}
\newcommand{\st}{\t{s.t.}}

\newcommand{\etal}{\textit{et al}. }


\newcommand{\pe}[1]{{\color{blue} \textrm{PE: #1}}}
\newcommand{\gs}[1]{{\color{red} \textrm{GS: #1}}}
\newcommand{\imr}[1]{{\color{cyan} \textrm{IMR: #1}}}

\newcommand{\rag}[1]{{\color{magenta} \textrm{RKR: #1}}}
\newcommand{\new}[1]{{\color{blue} \textrm{#1}}}

\renewcommand{\v}{\boldsymbol}
\renewcommand{\t}[1]{{\textrm{#1}}}

\newcommand{\R}{\mathbb{R}}
\newcommand{\data}{\mathcal{D}}

\newcommand{\eq}{Equation~} 
\newcommand{\eqs}{Equations~}
\newcommand{\fig}{Figure~}
\newcommand{\alg}{Algorithm~}
\newcommand{\algs}{Algorithms~}
\newcommand{\sect}{Section~}
\newcommand{\cha}{Chapter~}
\newcommand{\tab}{Table~}

\newcommand{\opt}{^\star}

\ifdefined\T
\renewcommand{\T}{^\top}
\else
\newcommand{\T}{^\top}
\fi

\newcommand{\mat}[3][.9]{
  \renewcommand{\arraystretch}{#1}{\scriptscriptstyle{\left(
    \hspace*{-1ex}\begin{array}{#2}#3\end{array}\hspace*{-1ex}
  \right)}}\renewcommand{\arraystretch}{1.2}
}

\newcommand{\bmat}[3][.9]{
  \renewcommand{\arraystretch}{#1}{\scriptscriptstyle{\left[
    \hspace*{-1ex}\begin{array}{#2}#3\end{array}\hspace*{-1ex}
  \right]}}\renewcommand{\arraystretch}{1.2}
}

\newcommand{\inv}{^{-1}}
\newcommand{\diag}{\text{diag}}

\newcommand{\comma}{~,}
\newcommand{\period}{~.}

\newcommand{\ga}{\alpha}
\newcommand{\gb}{\beta}
\newcommand{\gd}{\delta}
\newcommand{\gD}{\Delta}
\renewcommand{\ge}{\epsilon}
\renewcommand{\gg}{\gamma}
\newcommand{\gG}{\Gamma}
\newcommand{\gl}{\lambda}
\newcommand{\gL}{\Lambda}
\newcommand{\gm}{\mu}
\newcommand{\gn}{\nu}
\newcommand{\gN}{\nabla}
\newcommand{\gk}{\kappa}
\newcommand{\go}{\omega}
\newcommand{\gO}{\Omega}
\newcommand{\gp}{\phi}
\newcommand{\gph}{\varphi}
\newcommand{\gP}{\Phi}
\newcommand{\gr}{\rho}
\newcommand{\grh}{\varrho}
\newcommand{\gsi}{\sigma}
\newcommand{\gSi}{\Sigma}
\newcommand{\gt}{\theta}
\newcommand{\gT}{\Theta}
\newcommand{\gv}{\vartheta}
\newcommand{\gx}{\xi}
\newcommand{\gX}{\Xi}
\newcommand{\gY}{\Upsilon}
\newcommand{\gz}{\zeta}

% math environments
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{theorem}{Theorem}

\newcommand{\lemmaautorefname}{Lemma}
\newcommand{\algorithmautorefname}{Algorithm}

==> related_work.tex <==
\section{Related work}
\label{sec:related_work}
% TODO: move any related work to the intro, cut down on CSBMP and include more manifold learning. 

\subsection{Constrained SBMP} \label{csbmp} Sampling-based motion planning
(SBMP) is a broad field which tackles the problem of motion planning by using
randomized sampling techniques to build a tree or graph of configurations (also
called samples). The resulting tree or graph can then be used to plan paths
between configurations. This is in contrast to other motion planning techniques,
which may optimize an objective function over a continuous space of trajectories
(e.g., \citet{kalakrishnan2011stomp}) or use the gradient of a potential field
to guide a path toward a goal configuration (e.g., \citet{khatib1986real}).
Many SBMP algorithms derive from one of the following SBMP methods:
Rapidly-exploring random tree (RRT) (\citet{lavalle1998rapidly,
lavalle2006planning}), probabilistic roadmap (PRM)
(\citet{kavraki1994randomized}), and their optimal counterparts RRT* and PRM*
(\citet{karaman2011sampling}). These methods work by sampling the search space,
connecting samples if the edge between them does not collide with obstacles, and
then querying the tree or graph for a valid path that reaches the goal state. A
collision detector is generally assumed to exist, which reports whether or not a
state is in collision with obstacles in the environment. 

A more challenging and realistic motion planning task is that of constrained
SBMP, where there are motion constraints beyond simply obstacle avoidance.
Constraints will often lead to a free configuration space manifold $C_{free} \in
\mathbb{R}^{d'}$ of lower dimension than the ambient configuration space $C \in
\mathbb{R}^d$. (For example, consider the constraint where an arm must stay at a
particular height. A joint that moves the arm up and down will have an effective
space of only one value, and hence the rest of the configuration space is
"squashed" down a dimension.) Randomized sampling in a $d$-dimensional space
will produce samples on a $d' < d$ -dimensional space with probability 0, so
additional measures must be taken to produce valid samples for planning. Another
complication arises when there is not just one constraint, but many, which may
have a specific order in which they must be met in order to achieve the task
goal.

\subsection{Manifold Learning}

==> use_in_planning.tex <==
\section{Use in planning}
\label{sec:use_in_planning}
